LC-Score: Reference-less estimation of Text Comprehension Difficulty

Being able to read and understand written text is critical in a digital era. However, studies shows that a large fraction of the population experiences comprehension issues. In this context, further initiatives in accessibility are required to improve the audience text comprehension. However, writers are hardly assisted nor encouraged to produce easy-to-understand content. Moreover, Automatic Text Simplification (ATS) model development suffers from the lack of metric to accurately estimate comprehension difficulty We present \textsc{LC-Score}, a simple approach for training text comprehension metric for any French text without reference \ie predicting how easy to understand a given text is on a $[0, 100]$ scale. Our objective with this scale is to quantitatively capture the extend to which a text suits to the \textit{Langage Clair} (LC, \textit{Clear Language}) guidelines, a French initiative closely related to English Plain Language. We explore two approaches: (i) using linguistically motivated indicators used to train statistical models, and (ii) neural learning directly from text leveraging pre-trained language models. We introduce a simple proxy task for comprehension difficulty training as a classification task. To evaluate our models, we run two distinct human annotation experiments, and find that both approaches (indicator based and neural) outperforms commonly used readability and comprehension metrics such as FKGL.

==> cmd/pltrdy_commands.tex <==
% For commands without arguments, e.g. \latin
% https://tex.stackexchange.com/a/31092/150208
\usepackage{xspace}

% Mise en forme
\newcommand{\bs}{\textbackslash}
\newcommand{\code}[1]{\texttt{#1}}

\newcommand{\nom}[1]{\textsc{#1}}
\newcommand{\model}[1]{\textsc{#1}}
\newcommand{\critere}[1]{#1}
\newcommand{\dataset}[1]{\texttt{\small{#1}}}

\newcommand{\latin}[1]{\textit{#1}\xspace}
\newcommand{\ie}{\latin{i.e.}}
\newcommand{\eg}{\latin{e.g.}}
\newcommand{\etc}{\latin{etc.}}

\newcommand{\cf}{\latin{cf.}}

\newcommand{\best}[1]{{\boldmath\bfseries#1}}

\newcommand{\trad}[1]{\textit{#1}}
\newcommand{\abrv}[1]{\textit{#1}}

% List title when e.g. \item \listemph{Item}~: description
\newcommand{\listemph}[1]{\textbf{#1}}
\newcommand{\lemph}[1]{\listemph{#1}}

% Models & Datasets (alias for compatibility)
\newcommand{\modelname}[1]{\model{#1}}
\newcommand{\datasetname}[1]{\dataset{#1}}
\newcommand{\publicmeetings}{\texttt{\small{public\_meetings}}\xspace}

\newcommand{\warning}[1]{{\PackageWarning{pltrdy_commands}{#1}}}
% \newcommand{\warning}[1]{#1}

% Special paragraphs
% \usepackage{xcolor}[dvipsnames]
% \newcommand{\todo}[1]{{{\ttodo{#1}}{\warning{TODO}}}}
\newcommand{\todo}[1]{{\color{red}[\textbf{\underline{TODO:}} #1]} \warning{TODO}} % \warning{TODO: #1}
\newcommand{\bettertrad}[1]{{\color{red}[\textbf{\underline{Better Trad:}} #1]} \warning{Better TRAD: #1}} % \warning{TODO: #1}
\newcommand{\notes}[1]{{\color{blue}[\textbf{\underline{NOTES:}} #1] \warning{NOTES}}}% \warning{There's still NOTES}}
\newcommand{\missingref}[1]{{\textcolor{purple}{#1 (\textbf{\underline{Missing ref!}})}\warning{MissingRef: #1}}} % \warning{NoRef: #1}}
% \newcommand{\idea}[1]{\textcolor{green}{\textbf{\underline{IDEA:}} #1}}
\newcommand{\idea}[1]{{\textcolor{ForestGreen}{\textbf{\underline{IDEA:}} #1} \warning{IDEA}}}% \warning{There's still IDEA}}

%\newcommand{\warning}[1]{{\message{LaTeX Warning: \noexpand #1 \the\inputlineno}}}
%\newcommand{\warning}[1]{{\PackageError{pltrdy_warnings}{#1}{\the\inputlineno}}}

% French quotes
% https://tex.stackexchange.com/a/541077/150208
\usepackage{csquotes}
\MakeOuterQuote{"}


% Chapter Table of content with minitoc
% https://tex.stackexchange.com/a/3002/150208
\usepackage{minitoc}

% Replace "Contents" in minitoc title by translation
% https://tex.stackexchange.com/a/312981/150208
\addto{\captionsfrench}{% Making babel aware of special titles
  \renewcommand{\mtctitle}{Table des matières}
}

% Custom chapter command with minitoc

\newcommand{\dochapter}[2]{%
    \chapter{#1}
    #2%
    \vfill
    \minitoc%
    \clearpage%
}

% Cleveref 
% like autoref but with capitalization
% https://tex.stackexchange.com/a/34160/150208
% \usepackage{listings}
% \usepackage[nameinlink]{cleveref}

% Extending autoref with Autoref for capitalization
% \usepackage{catoptions}
% \makeatletter
% \def\figureautorefname{figure}
% \def\tableautorefname{tableau}
% \def\Autoref#1{%
%   \begingroup
%   \edef\reserved@a{\cpttrimspaces{#1}}%
%   \ifcsndefTF{r@#1}{%
%     \xaftercsname{\expandafter\testreftype\@fourthoffive}
%       {r@\reserved@a}.\\{#1}%
%   }{%
%     \ref{#1}%
%   }%
%   \endgroup
% }
% \def\testreftype#1.#2\\#3{%
%   \ifcsndefTF{#1autorefname}{%
%     \def\reserved@a##1##2\@nil{%
%       \uppercase{\def\ref@name{##1}}%
%       \csn@edef{#1autorefname}{\ref@name##2}%
%       \autoref{#3}%
%     }%
%     \reserved@a#1\@nil
%   }{%
%     \autoref{#3}%
%   }%
% }
% \makeatother
%%%%%%%%%%%%%%%%%%%



% Enumeration, allows e.g.\begin{enumerate}[label=\alph*] for small letters
% shortlabels: labels as an example \eg \begin{enumerate}[(1)]
\usepackage[shortlabels]{enumitem}

% \begin{enumerate}[i]
% \usepackage{enumerate}


% landscape 
% https://tex.stackexchange.com/a/19021/150208
% \usepackage{pdflscape}
% \usepackage{afterpage}

% check and cross symbol     
% https://tex.stackexchange.com/questions/42619/x-mark-to-match-checkmark
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\nmark}{--}%

%%%%%%%%%% Tables 
%%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%%
% Thick/Thin separator in tables
% https://tex.stackexchange.com/a/3449/150208
\usepackage{booktabs}
% \setlength{\arrayrulewidth}{0.05em}
% \setlength{\heavyrulewidth}{0.08em}
% \setlength{\lightrulewidth}{0.08em}
% \setlength{\heavyrulewidth}{0.15em}
% \newcommand{\submidrule}{\midrule[0.01em]}
\setlength{\lightrulewidth}{0.08em}
\setlength{\heavyrulewidth}{0.10em}
\newcommand{\submidrule}{\midrule[0.0em]}

\usepackage{ctable} % for \specialrule command
\newcommand{\hthinline}{\specialrule{.0005em}{.25em}{.25em}}

% Custom table cells
% see https://tex.stackexchange.com/questions/2441/how-to-add-a-forced-line-break-inside-a-table-cell/19678
% \usepackage{fourier} 
\usepackage{array}
\usepackage{makecell}
\usepackage{float}
\renewcommand\theadalign{bc}
% \renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}
\newcommand{\subhead}[2]{\thead{\textbf{#1} \\ #2}}

% y is supposed to be even better than x:
% https://en.wikibooks.org/wiki/LaTeX/Tables#The_tabulary_package
% \usepackage{tabulary}


% for wraping text in table
% https://stackoverflow.com/questions/790932/how-to-wrap-text-in-latex-tables
\usepackage{tabularx}
% Y = centered X
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}

% dashed mid rule
% https://tex.stackexchange.com/a/169103/150208
\usepackage{arydshln}
% \setlength\dashlinedash{0.2pt}
% \setlength\dashlinegap{1.5pt}
% \setlength\arrayrulewidth{0.3pt}



% increase row height w/ vertical centering
% https://tex.stackexchange.com/a/483011/150208
\usepackage{stackengine}
\newcommand\xrowht[2][0]{\addstackgap[.5\dimexpr#2\relax]{\vphantom{#1}}}

% Multirow
% https://tex.stackexchange.com/a/72972/150208
\usepackage{multirow}

% Sideway table
\usepackage{rotating}

% Imported below, in section "figures" w/ option "export", ignoring here.
% \usepackage{adjustbox}
%%%

%%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%%


% Bold abbreviation for best score in table
\newrobustcmd{\B}{\bfseries}

% Best line, best row
\newrobustcmd{\Bl}{}%\B}
\newrobustcmd{\Br}{}%\B}

% missing result in table (to be computed)
\newrobustcmd{\MR}{{\color{red}\textbf{??}}}
% missing result in table (just need to be reported)
\newrobustcmd{\TR}{{\color{blue}\textbf{!?}}}

% external results
\newrobustcmd{\extRes}[1]{\emph{#1}}
\newrobustcmd{\extResA}[1]{\extRes{#1\textsuperscript{*}}}
\newrobustcmd{\extResB}[1]{\extRes{#1\textsuperscript{$\star$}}}
\newrobustcmd{\extResC}[1]{\extRes{#1\textsuperscript{$\circ$}}}

%%%%%%%%%% Figures 
%%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%%
% taille de figure i.e. \textwidth
% https://tex.stackexchange.com/questions/37790/scale-figure-to-a-percentage-of-textwidth
\usepackage{graphicx}

% allow H positioning, stronger than !h
\usepackage{float} 

% \includegraphics[max width=\textwidth]{some_image_in_pdf.pdf}
% + adjust table w/
% \adjustbox{max width=\textwidth}{
%   \begin{table}[!htbp]
%    ...
% }
\usepackage[export]{adjustbox}% http://ctan.org/pkg/adjustbox

% Subfigures
% https://tex.stackexchange.com/questions/37581/latex-figures-side-by-side
\usepackage{caption}
\usepackage{subcaption}

% Subfigures (not side by side)
\usepackage{subfloat}
%%%
%%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%%

%%%%%%%%%% Tikz 
%%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%%
\usepackage{tikz}

% For "Computer Modern Rightarrow" e.g. LREC alignment figure
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
% /!\ subfig incompatible w/ subcaption
% \usepackage{subfig}
%%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%%



%%%%%%%%%% Math notations 
%%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%%

% For mathbbm, in particular, $\mathbbm{1}$ is usefull for "1 if condition 0 else"
\usepackage{bbm}

\def\ystar{{y^{*}}}
\def\yhat{{\hat{y}}}

\def\astar{{a^{*}}}
\def\ahat{{\hat{a}}}

\def\lstar{{l^{*}}}
\def\lhat{{\hat{l}}}

\def\tstar{{t^{*}}}
\def\that{{\hat{t}}}
%%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%%

\usepackage{boxedminipage} % for the examples in figures


%%%%%%%%%% Appendices 
%%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%% %%%%%%%%%%
\usepackage[toc,page]{appendix}
\renewcommand{\appendixname}{Annexe}
\renewcommand{\appendixpagename}{Annexes}
\renewcommand{\appendixtocname}{Annexes}

% Fix autoref w/ Appendix
% https://tex.stackexchange.com/a/299687/150208
\makeatletter
\addto\extrasfrench{%
  % \renewcommand{\chapterautorefname}{Kapitel}%
  \renewcommand{\appendixautorefname}{\appendixname}%
   \renewcommand{\tableautorefname}{tableau}%
   \renewcommand{\figureautorefname}{figure}%
%   \@ifundefined{Annexeautorefname}{%
%     \newcommand{\AAnnexeautorefname}{\appendixname}%
%   }{%
%     \renewcommand{\Annexeautorefname}{\appendixname}%
%   }
% Use "section" for sub- and sub-sub- sections autoref
    \renewcommand{\subsectionautorefname}{\sectionautorefname}
    \renewcommand{\subsubsectionautorefname}{\sectionautorefname}
    \renewcommand{\bibname}{Bibliographie}
}

\makeatother

% Use "section" for sub- and sub-sub- sections autoref
\let\subsectionautorefname\sectionautorefname
\let\subsubsectionautorefname\sectionautorefname

==> cmd/pltrdy_math_commands.tex <==
%% Commands defined during BILAN2018, mostly for defining models etc

% Ajouté pour \llbracket et \\rrbracket (intervalles d'entiers)
\usepackage{stmaryrd}

\usepackage{amsmath,amsfonts,bm}

% declaring vectors \vx to be \vect{x}
% src: https://tex.stackexchange.com/questions/83939/new-command-based-on-command-name
\newcommand{\boldvector}[1]{{\bm{#1}}}
\newcommand{\bv}[1]{\boldvector{#1}}

% \newcommand{\bs}[1]{\boldsymbol{#1}}

\makeatletter
\@tfor\next:=abcdefghijklmnopqrstuvwxyxzABCDEFGHIJKLMNOPQRSTUVWXYZ\do
 {\begingroup\edef\x{\endgroup
    \noexpand\@namedef{v\next}{\noexpand\boldvector{\next}}%
  }\x}

\newcommand{\boldmatrix}[1]{\mathbf{#1}}
% NOTE: u is excluded to keep the greek letter \mu
\@tfor\next:=abcdefghijklmnopqrstvwxyxzABCDEFGHIJKLMNOPQRSTUVWXYZ\do
 {\begingroup\edef\x{\endgroup
    \noexpand\@namedef{m\next}{\noexpand\boldmatrix{\next}}%
  }\x}


\newcommand{\mathdataset}[1]{{\mathcal{#1}}}
\@tfor\next:=abcdefghijklmnopqrstuvwxyxzABCDEFGHIJKLMNOPQRSTUVWXYZ\do
 {\begingroup\edef\x{\endgroup
    \noexpand\@namedef{ds\next}{\noexpand\mathdataset{\next}}%
  }\x}
\makeatother
% ------------

% declaring embedding vectors
% src: https://tex.stackexchange.com/questions/83939/new-command-based-on-command-name
% NOTE 2021-02-09 : removing tilde, is not clear
\newcommand{\embvector}[1]{\bv{#1}}
\newcommand{\Embvector}[1]{\boldmatrix{#1}}

\makeatletter
\@tfor\next:=abcdefghijklmnopqrstuvwxyxz\do
 {\begingroup\edef\x{\endgroup
    \noexpand\@namedef{emb\next}{\noexpand\embvector{\next}}%
  }\x}
\makeatother


% Old embedding
\newcommand{\oldembvector}[1]{\Tilde{\bv{#1}}\warning{Use of oldembvector deprecated}}
\makeatletter
\@tfor\next:=abcdefghijklmnopqrstuvwxyxz\do
 {\begingroup\edef\x{\endgroup
    \noexpand\@namedef{oldemb\next}{\noexpand\oldembvector{\next}}%
  }\x}
\makeatother

% Tilde vector
\newcommand{\tildevector}[1]{\Tilde{\bv{#1}}}
\makeatletter
\@tfor\next:=abcdefghijklmnopqrstuvwxyxz\do
 {\begingroup\edef\x{\endgroup
    \noexpand\@namedef{tv\next}{\noexpand\tildevector{\next}}%
  }\x}
\makeatother


\makeatletter
\@tfor\next:=abcdefghijklmnopqrstuvwxyxz\do
 {\begingroup\edef\x{\endgroup
    \noexpand\@namedef{Emb\next}{\noexpand\Embvector{\next}}%
  }\x}
\makeatother

% declaring bar vectors
\newcommand{\barvector}[1]{\overline{{#1}}}

\makeatletter
\@tfor\next:=abcdefghijklmnopqrstuvwxyxz\do
 {\begingroup\edef\x{\endgroup
    \noexpand\@namedef{bar\next}{\noexpand\barvector{\next}}%
  }\x}
\makeatother


% dimensions prefix d_
\newcommand{\dimension}[1]{d_{#1}}

\def\demb{{\dimension{emb}}}
\def\denc{{\dimension{enc}}}
\def\ddec{{\dimension{dec}}}
\def\dgen{{\dimension{gen}}}



\newcommand\Chapter[2]{\chapter
  [#1\hfil\hbox{}\protect\linebreak{\itshape#2}]%
  {#1\\[2ex]\Large\itshape#2}%
}

%% -----------------------------------------

% vocabulary
\def\vocab{{\mathcal{V}}}

% transpose 
\newcommand{\T}{^{\top}}

% Commands for Paulus
\newcommand{\ypred}{\hat y}
\newcommand{\ys}{y^{s}}
\newcommand{\ytgt}{y}

\newcommand{\Vx}{{\mathcal{V}_{x}}}
\newcommand{\Vy}{{\mathcal{V}_{y}}}
\newcommand{\Vytgt}{{\mathcal{V}_{\ytgt}}}
\newcommand{\Vsx}{{V_{x}}}
\newcommand{\Vsy}{{V_{y}}}
\newcommand{\Vsytgt}{{V_{\ytgt}}}

\newcommand{\Tx}{{\card{x}}}
\newcommand{\Ty}{{\card{y}}}
\newcommand{\Tytgt}{{\card{\ytgt}}}

\newcommand{\Ex}{{\mathbf{E}_{x}}}
\newcommand{\Ey}{{\mathbf{E}_{y}}}
\newcommand{\Ectx}{{\mathbf{E}_{c}}}
\newcommand{\Esx}{{D_{x}}}
\newcommand{\Esy}{{D_{y}}}

\newcommand{\hd}{\bv{h}^d}
\newcommand{\he}{\bv{h}^e}
\newcommand{\cd}{\bv{c}^d}
\newcommand{\ce}{\bv{c}^e}
\newcommand{\ed}{\bv{e}^d}
\newcommand{\ee}{\bv{e}^e}
\newcommand{\etmp}{\bv{e}^{tmp}}

\newcommand{\alphae}{\alpha^e}
\newcommand{\alphad}{\alpha^d}

\newcommand{\Wattn}{\mW_{attn}}
\newcommand{\Wae}{\Wattn^e}
\newcommand{\Wad}{\Wattn^d}

\newcommand{\Vattn}{\mV_{attn}}
\newcommand{\Vae}{\Vattn^e}

\newcommand{\Hd}{\boldvector{h}^d}
\newcommand{\He}{\boldvector{h}^e}
\newcommand{\Cd}{\boldvector{c}^d}
\newcommand{\Ce}{\boldvector{c}^e}

\newcommand{\Wout}{\mW_{out}}
\newcommand{\bout}{b_{out}}
\newcommand{\Vout}{\mV_{out}}
\newcommand{\boutp}{b_{{out}^\prime}}

\newcommand{\pgen}{p_{gen}}

\newcommand{\fwd}[1]{{\overrightarrow{#1}}}
\newcommand{\bwd}[1]{{\overleftarrow{#1}}}
\newcommand{\vfwd}[1]{{\fwd{#1}}}
\newcommand{\vbwd}[1]{{\bwd{#1}}}

% Empty set
% https://tex.stackexchange.com/a/22799/150208
\let\oldemptyset\emptyset
\let\emptyset\varnothing
%%%

% Loss
\newcommand{\Loss}{\mathcal{L}}
\newcommand{\loss}{\Loss}
%%%

% Functions
% \DeclareMathOperator*{\softmax}{\mathrm{softmax}}
\DeclareMathOperator*{\attention}{\mathrm{attention}}
\DeclareMathOperator*{\ROUGE}{\mathrm{ROUGE}}
%\DeclareMathOperator*{\ROUGE1}{\mathrm{ROUGE-1}}
%\DeclareMathOperator*{\ROUGE2}{\mathrm{ROUGE-2}}
%\DeclareMathOperator*{\ROUGE3}{\mathrm{ROUGE-3}}
%\DeclareMathOperator*{\ROUGEL}{\mathrm{ROUGE-L}}
% \DeclareMathOperator*{\sigmoid}{\mathrm{sigmoid}}
% \DeclareMathOperator*{\encoder}{\mathrm{encoder}}
% \DeclareMathOperator*{\decoder}{\mathrm{decoder}}

\DeclareMathOperator{\encoder}{\mathrm{encodeur}}
\DeclareMathOperator{\decoder}{\mathrm{decodeur}}
\newcommand{\Encoder}[1]{\encoder\left(#1\right)}
\newcommand{\Decoder}[1]{\decoder\left(#1\right)}

\newcommand{\activation}{\varphi}
\newcommand{\Activation}[1]{\activation\left(#1\right)}

\DeclareMathOperator{\dualxent}{dual\_xent}
\DeclareMathOperator{\entropy}{H}
\DeclareMathOperator{\ppl}{ppl}

\def\argmax{\operatornamewithlimits{arg\,max}}

\usepackage{mathtools}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\newcommand{\card}[1]{\abs*{ #1 }}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LREC2020 commands
% Custom math variables / function
\DeclareMathOperator{\score}{\mathit{score}}

% Documents, capitalized, mathcal
\def\Tr{{\mathcal{T}}}
\def\Rep{{\mathcal{R}}}
\def\lenTr{{\card{\Tr}}}
\def\lenRep{{\card{\Rep}}}

\def\TrS{{\hat{\mathcal{T}}}}
\def\RepS{{\hat{\mathcal{R}}}}
\def\lenTrS{{\card{\TrS}}}
\def\lenRepS{{\card{\RepS}}}

\def\oneif{{\mathbbm{1}}}

% Segments, capitalized (set of sentence)
\def\tseg{{\mathit{T}}}
\def\rseg{{\mathit{R}}}
\def\tsen{{\mathit{t}}}
\def\rsen{{\mathit{r}}}
% sentence
\DeclareMathOperator{\sen}{s}

% Alignment:
\DeclareMathOperator{\alignmentfct}{\mathit{alignement}} % alignment function

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tokens commands
% Custom math variables / function
% \newcommand{\tok}[1]{#1}
% \newcommand{\tok}[1]{#1}

% \newcommand{\up}[1]{\textsuperscript{#1}}

% Change mathcal mathscr
% https://tex.stackexchange.com/questions/349321/using-the-stix-font-for-mathcal-and-mathscr-only
\makeatletter
\DeclareFontEncoding{LS1}{}{}
\DeclareFontEncoding{LS2}{}{\noaccents@}
\DeclareFontSubstitution{LS1}{stix}{m}{n}
\DeclareFontSubstitution{LS2}{stix}{m}{n}
\makeatother

\DeclareMathAlphabet\mathscr{LS1}{stixscr}{m}{n}
% \SetMathAlphabet\mathscr{bold}{LS1}{stixscr}{b}{n}
\DeclareMathAlphabet\mathcal{LS2}{stixcal}{m}{n}
% \SetMathAlphabet\mathcal{bold}{LS2}{stixcal}{b}{n}
%%%


% Math operators

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\round}{round\,to}

% Ceil and Floor : 
% https://tex.stackexchange.com/a/118217/150208
\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% Logique
\let\implies\relax\DeclareMathOperator{\implies}{\Rightarrow}
\DeclareMathOperator{\equivalent}{\Leftrightarrow}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Gradient
\def\grad{{\nabla}}

% Follow distribution
\def\follow{{\sim}}

% Correlation
\def\pearson{{r}}
\def\spearman{{\rho}}
\def\fleiss{{\kappa}}

% Variation coeficient i.e. \sigma / \mu
\def\varcoef{{c_v}}

% Hadamard product
% \def\hprod{{\odot}}
\DeclareMathOperator{\hprod}{\odot}

% placeholder for function parameter 
% i.e. f(\argdot, \argdot) 
\def\argdot{{\hspace{0.18em}\cdot\hspace{0.18em}}}

% Phantom for equation alignment 
% https://tex.stackexchange.com/a/448386/150208
\newcommand*\phantomrel[1]{\mathrel{\phantom{#1}}}

% 
\newcommand{\bigO}{\mathcal{O}}

